Zonal asymmetries control the response of atmospheric blocking to Arctic warming in an aquaplanet experiment

In recent years a weak but robust response of mean midlatitude circulation to Arctic amplification (AA) has emerged from modeling experiments. However, open questions remain about the mechanisms linking such circulation differences to weather extremes in the midlatitudes. In this study we investigate such mechanisms and the importance of zonal asymmetries in shaping the atmospheric blocking response to AA. We perform idealized aquaplanet simulations in two configurations: a zonally symmetric setup and a zonally asymmetric experiment featuring a localized midlatitude storm track. For each configuration, we examine the response to AA by imposing an anomalous surface heating in the polar region. In the zonally symmetric configuration atmospheric blocking increases uniformly with AA from mid to high latitudes. In the asymmetric configuration, the response is more complex; instead of a zonally uniform response, we observe an upstream displacement of the blocking maximum, which sits at the exit of the localized storm track. We interpret these changes through the lens of the Traffic Jam theory by diagnosing the carrying capacity of the midlatitude flow. In both configurations, the zonally averaged increase in blocking is primarily driven by a weakening of the zonal winds, which reduces the Doppler-shifted Rossby wave group velocity and, in turn, decreases the flow carrying capacity. While the reduction in carrying capacity has similar characteristics in the two configurations, in the asymmetric case it leads to an upstream shift of blocking frequency as a direct consequence of the threshold behavior of blocking onset that lies at the core of the Traffic Jam theory. This mechanism, which has received limited attention so far, highlights the importance of mean circulation characteristics in shaping the blocking response to external forcing such as Arctic warming.

==> correlations_table.tex <==
\begin{table}
    \centering
    \begin{tabular}{|c|c|c|c|} \hline 
         /&  GHA&  GHA upstream& GHA retrograding\\ \hline 
         DAV&  0.20&  0.11& 0.15\\ \hline 
         DAV upstream&  0.11&  0.12& 0.05\\ \hline 
         DAV retrograding&  0.13&  0.05& 0.15\\ \hline
    \end{tabular}
    \caption{Jaccard coefficients for the Boolean time-series produced through the DAV and GHA indices. GHA and DAV refer to the time series of blocked and non-blocked days in the Greenland region, the suffix 'upstream' refers to the time-series where only upstream blocks are retained and the suffix 'retrograding' refers to the time-series where only retrograding blocks are retained. For the details on how the coefficient has been computed see the Methods section.}
    \label{jaccard}
\end{table}

In Table \ref{jaccard} we show the Jaccard coefficient of the boolean time series obtained through the different blocking indices. It is evident how the coefficients assume very small values for all the combination (1 = highly correlated, 0 = uncorrelated). This low correlation is motivated by the fact that blocking occurs rarely and when it occurs the different indices identify blockings in different areas and at different stages of its life-cycle. Yet, Table \ref{jaccard} contains some useful information. In order to confirm that such correlations are not random we note that the combinations (GHA upstream, DAV retrograding) and (GHA retrograding, DAV upstream) are very little correlated, as expected. Moreover, it is possible to notice that the maximum correlation are obtained when considering all the events (DAV, GHA) or when considering the retrograding events (DAV retrograding, GHA retrograding), while the upstream events are less correlated. This further sustain the idea that upstream events are Omega blocks that can develop into Rex blocks. The GHA index struggles with detecting Rex blocks and the intrusion of polar air from higher latitudes, while the DAV index struggles with detecting Omega blocks, resulting in a weaker correlation between the two. Conversely, retrograding blocks consist in breaking Rossby waves that can be effectively detected by both indices, resulting in a slightly higher correlation.

